Frequency and mode identification of {\gamma} Doradus from photometric and spectroscopic observations

The prototype star for the {\gamma} Doradus class of pulsating variables was studied em- ploying photometric and spectroscopic observations to determine the frequencies and modes of pulsation. The four frequencies found were self-consistent between the obser- vation types and almost identical to those found in previous studies (1.3641 d-1 ,1.8783 d-1 , 1.4742 d-1 and 1.3209 d-1). Three of the frequencies are classified as l, m = (1, 1) pulsations and the other is ambiguous between l = 2 modes. Two frequencies are shown to be stable over twenty years since their first identification. The agreement in ground-based work makes this star an excellent calibrator for the upcoming TESS observations and a standard for continued asteroseismic modelling.

==> subfigure.tex <==
%%
%% This is file `subfigure.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% subfigure.dtx  (with options: `package')
%% 
%% Copyright (C) 1986-2002 Steven Douglas Cochran.
%% 
%% This file is NOT the source for subfigure, because almost all comments
%% have been stripped from it.  It is NOT the preferred form of subfigure
%% for making modifications to it.
%% 
%% Therefore you can NOT redistribute and/or modify THIS file.  You can
%% however redistribute the complete source (subfigure.dtx and
%% subfigure.ins) and/or modify it under the terms of the LaTeX Project
%% Public License, either version 1.2 of this license or (at your option)
%% any later version. The latest version of this license is in:
%%      http://www.latex-project.org/lppl.txt
%% and version 1.2 or later is part of all distributions of LaTeX version
%% 1999/09/03 or later.
%% 
%% The subfigure package is distributed in the hope that it will be
%% useful, but WITHOUT ANY WARRANTY; without even the implied warranty of
%% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the LaTeX
%% Project Public License for more details.
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% @LaTeX-style-file{
%%    author     = "Steven Douglas Cochran",
%%    version    = "2.1.5",
%%    date       = "2005/04/29",
%%    time       = "14:24:08",
%%    filename   = "subfigure.sty",
%%    address    = "Digital Mapping Laboratory, School of Computer Science
%%                  Carnegie-Mellon University, 5000 Forbes Avenue
%%                  Pittsburgh, PA 15213-3890, USA",
%%    telephone  = "+1 412.268.5654",
%%    fax        = "+1 412.268.5576",
%%    email      = "cochran@ieee.org",
%%    codetable  = "ISO/ASCII",
%%    keywords   = "LaTeX, float, figure, table, captcont",
%%    supported  = "yes",
%%    abstract   = "LaTeX package for providing support for the
%%                  inclusion of small, `sub', figures and tables.  It
%%                  simplifies the positioning, captioning and
%%                  labeling of them within a single figure or table
%%                  environment.  In addition, this package allows
%%                  such subcaptions to be written to the List of
%%                  Figures or List of tables if desired."
%% }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1994/12/01]
\ProvidesPackage{subfigure}[2002/03/15 v2.1.5 subfigure package]
\def\sf@floatfix#1#2{%
  \ifx#1#2%
    \ifx#1\@undefined\else
      \PackageWarningNoLine{subfigure}{%
Your document class has a bad definition^^J
of \string#1, most likely^^J
\string\let\string#1=\string#2^^J
which has now been changed to^^J
\string\def\string#1{\string#2}^^J
because otherwise subsequent changes to \string#2^^J
(like done by several packages changing float behaviour)^^J
can't take effect on \string#1.^^J
Please complain to your document class author}%
      \def#1{#2}%
    \fi
  \fi}
\begingroup
\def\next#1#2{%
    \endgroup
  \sf@floatfix\endfigure{end@float}
  \sf@floatfix\endtable\end@float
  \sf@floatfix#1\end@dblfloat
  \sf@floatfix#2\end@dblfloat}
\expandafter\next\csname endfigure*\expandafter\endcsname
  \csname endtable*\endcsname
\newif\ifhyperrefloaded
\AtBeginDocument{%
  \@ifpackageloaded{hyperref}{%
    \hyperrefloadedtrue
    \providecommand\theHsubfigure{\thefigure.\arabic{subfigure}}%
    \providecommand\theHsubtable{\thetable.\arabic{subtable}}%
    \providecommand{\toclevel@subfigure}{1}%
    \providecommand{\toclevel@subtable}{1}}{}}
\newif\ifsubcaphang
\newif\ifsubcapcenter
\newif\ifsubcapcenterlast
\newif\ifsubcapnooneline
\newif\ifsubcapraggedright
\newskip\subfigtopskip     \subfigtopskip    =  5\p@
\newskip\subfigcapskip     \subfigcapskip    =  0\p@
\newdimen\subfigcaptopadj  \subfigcaptopadj  =  3\p@
\newskip\subfigbottomskip  \subfigbottomskip =  5\p@
\newdimen\subfigcapmargin  \subfigcapmargin  =  \z@
\newskip\subfiglabelskip   \subfiglabelskip  =  0.33em plus 0.07em minus 0.03em
\newcommand*{\subcapsize}{}
\newcommand*{\subcaplabelfont}{%
  \subcaplabelfont@f\subcaplabelfont@c\subcaplabelfont@s}
\newcommand*{\subcaplabelfont@f}{\fontfamily{\familydefault}\selectfont}
\newcommand*{\subcaplabelfont@c}{\fontseries{\seriesdefault}\selectfont}
\newcommand*{\subcaplabelfont@s}{\fontshape{\shapedefault}\selectfont}
\newcommand*{\subcapfont}{%
  \subcapfont@f\subcapfont@c\subcapfont@s}
\newcommand*{\subcapfont@f}{\fontfamily{\familydefault}\selectfont}
\newcommand*{\subcapfont@c}{\fontseries{\seriesdefault}\selectfont}
\newcommand*{\subcapfont@s}{\fontshape{\shapedefault}\selectfont}
\newif\ifsf@tight          \sf@tighttrue
\newcounter{subfigure}[figure]
\@ifundefined{figuretopcaptrue}{\newif\iffiguretopcap}{}
\newif\ifsubfiguretopcap
\let\p@subfigure=\thefigure
\providecommand*{\thesubfigure}{(\alph{subfigure})}
\renewcommand*{\thesubfigure}{(\alph{subfigure})}
\newcommand*{\@thesubfigure}{\thesubfigure\hskip\subfiglabelskip}
\newcommand*{\@@thesubfigure}{\thesubfigure}
\let\ext@subfigure=\ext@figure
\newcommand*{\l@subfigure}{%
  \@dottedxxxline{\ext@subfigure}{2}{3.8em}{2.5em}}
\newcounter{lofdepth}
\setcounter{lofdepth}{1}
\newcounter{subtable}[table]
\@ifundefined{tabletopcaptrue}{\newif\iftabletopcap}{}
\newif\ifsubtabletopcap
\let\p@subtable=\thetable
\providecommand*{\thesubtable}{(\alph{subtable})}
\renewcommand*{\thesubtable}{(\alph{subtable})}
\newcommand*{\@thesubtable}{\thesubtable\hskip\subfiglabelskip}
\newcommand*{\@@thesubtable}{\thesubtable}
\let\ext@subtable=\ext@table
\newcommand*{\l@subtable}{%
  \@dottedxxxline{\ext@subtable}{2}{3.8em}{2.5em}}
\newcounter{lotdepth}
\setcounter{lotdepth}{1}
\DeclareOption{normal}{%
  \subcaphangfalse
  \subcapcenterfalse
  \subcapcenterlastfalse
  \subcapnoonelinefalse
  \subcapraggedrightfalse}
\DeclareOption{hang}{\subcaphangtrue}
\DeclareOption{center}{\subcapcentertrue}
\DeclareOption{centerlast}{\subcapcenterlasttrue}
\DeclareOption{nooneline}{\subcapnoonelinetrue}
\DeclareOption{raggedright}{\subcapraggedrighttrue}
\DeclareOption{isu}{\ExecuteOption{hang}}
\DeclareOption{anne}{\ExecuteOption{centerlast}}
\DeclareOption{scriptsize}{\renewcommand*{\subcapsize}{\scriptsize}}
\DeclareOption{footnotesize}{\renewcommand*{\subcapsize}{\footnotesize}}
\DeclareOption{small}{\renewcommand*{\subcapsize}{\small}}
\DeclareOption{normalsize}{\renewcommand*{\subcapsize}{\normalsize}}
\DeclareOption{large}{\renewcommand*{\subcapsize}{\large}}
\DeclareOption{Large}{\renewcommand*{\subcapsize}{\Large}}
\DeclareOption{rm}{\renewcommand*{\subcaplabelfont@f}{\rmfamily}}
\DeclareOption{sf}{\renewcommand*{\subcaplabelfont@f}{\sffamily}}
\DeclareOption{tt}{\renewcommand*{\subcaplabelfont@f}{\ttfamily}}
\DeclareOption{md}{\renewcommand*{\subcaplabelfont@c}{\mdseries}}
\DeclareOption{bf}{\renewcommand*{\subcaplabelfont@c}{\bfseries}}
\DeclareOption{up}{\renewcommand*{\subcaplabelfont@s}{\upshape}}
\DeclareOption{it}{\renewcommand*{\subcaplabelfont@s}{\itshape}}
\DeclareOption{sl}{\renewcommand*{\subcaplabelfont@s}{\slshape}}
\DeclareOption{sc}{\renewcommand*{\subcaplabelfont@s}{\scshape}}
\DeclareOption{RM}{\renewcommand*{\subcapfont@f}{\rmfamily}}
\DeclareOption{SF}{\renewcommand*{\subcapfont@f}{\sffamily}}
\DeclareOption{TT}{\renewcommand*{\subcapfont@f}{\ttfamily}}
\DeclareOption{MD}{\renewcommand*{\subcapfont@c}{\mdseries}}
\DeclareOption{BF}{\renewcommand*{\subcapfont@c}{\bfseries}}
\DeclareOption{IT}{\renewcommand*{\subcapfont@s}{\itshape}}
\DeclareOption{SL}{\renewcommand*{\subcapfont@s}{\slshape}}
\DeclareOption{SC}{\renewcommand*{\subcapfont@s}{\scshape}}
\DeclareOption{UP}{\renewcommand*{\subcapfont@s}{\upshape}}
\DeclareOption{figbotcap}{\figuretopcapfalse}
\DeclareOption{figtopcap}{\figuretopcaptrue}
\DeclareOption{tabbotcap}{\tabletopcapfalse}
\DeclareOption{tabtopcap}{\tabletopcaptrue}
\DeclareOption{FIGBOTCAP}{\ExecuteOptions{figbotcap}\subfiguretopcapfalse}
\DeclareOption{FIGTOPCAP}{\ExecuteOptions{figtopcap}\subfiguretopcaptrue}
\DeclareOption{TABBOTCAP}{\ExecuteOptions{tabbotcap}\subtabletopcapfalse}
\DeclareOption{TABTOPCAP}{\ExecuteOptions{tabtopcap}\subtabletopcaptrue}
\DeclareOption{loose}{%
  \subfigtopskip    = 10\p@
  \subfigcapskip    = 10\p@
  \subfigcaptopadj  =  0\p@
  \subfigbottomskip = 10\p@
  \subfigcapmargin  = 10\p@
  \subfiglabelskip  =  0.33em
  \renewcommand*{\@thesubfigure}{\thesubfigure\space}
  \renewcommand*{\@thesubtable}{\thesubtable\space}
  \sf@tightfalse}
\DeclareOption{tight}{%
  \subfigtopskip    =  5\p@
  \subfigcapskip    =  0\p@
  \subfigcaptopadj  =  3\p@
  \subfigbottomskip =  5\p@
  \subfigcapmargin  =  \z@
  \subfiglabelskip  =  0.33em plus 0.07em minus 0.03em
  \renewcommand*{\@thesubfigure}{\thesubfigure\hskip\subfiglabelskip}
  \renewcommand*{\@thesubtable}{\thesubtable\hskip\subfiglabelskip}
  \sf@tighttrue}
\ExecuteOptions{normal,footnotesize,FIGBOTCAP,TABBOTCAP,loose}
\InputIfFileExists{subfigure.cfg}{%
  \typeout{****************************************^^J%
           * Local config file subfigure.cfg used *^^J%
           ****************************************}}{}
\ProcessOptions
\newcommand*{\subfigure}{%
  \bgroup
    \let\subfig@oldlabel=\label
    \let\label=\subfloat@label
    \@nameuse{if\@captype topcap}\else
      \advance\@nameuse{c@\@captype}\@ne
    \fi
    \refstepcounter{sub\@captype}%
    \@ifnextchar [%
      {\@subfigure}%
      {\@subfigure[\@empty]}}
\let\subtable=\subfigure
\def\@subfigure[#1]{%
    \@ifnextchar [%
      {\@subfloat{sub\@captype}[{#1}]}%
      {\@subfloat{sub\@captype}[\@empty{#1}][{#1}]}}
\newskip\subfig@top
\newskip\subfig@bottom
\long\def\@subfloat#1[#2][#3]#4{%
    \@tempcnta=1
    \ifsf@tight
      \if@minipage
        \@tempcnta=\z@
      \else\ifdim \lastskip=\z@ \else
        \@tempcnta=2
      \fi\fi
    \fi
    \@nameuse{if\@captype topcap}%
      \subfig@top=\subfigbottomskip
      \subfig@bottom=\subfigtopskip
    \else
      \subfig@top=\subfigtopskip
      \subfig@bottom=\subfigbottomskip
    \fi
    \leavevmode
    \setbox\@tempboxa \hbox{#4}%
    \@tempdima=\wd\@tempboxa
    \vtop\bgroup
      \vbox\bgroup
        \ifcase\@tempcnta
          \@minipagefalse
        \or
          \vspace{\subfig@top}%
        \or
          \ifdim \lastskip=\z@ \else
            \@tempskipb\subfig@top\relax\@xaddvskip
          \fi
        \fi
        \@nameuse{if#1topcap}%
          \ifx \@empty#3\relax \else
            \@subcaption{#1}{#2}{#3}%
            \vskip\subfigcapskip
            \vskip\subfigcaptopadj
          \fi\egroup
          \box\@tempboxa
        \else
          \box\@tempboxa\egroup
          \ifx \@empty#3\relax \else
            \vskip\subfigcapskip
            \@subcaption{#1}{#2}{#3}%
          \fi
        \fi
      \vspace{\subfig@bottom}%
    \egroup
    \@nameuse{if\@captype topcap}\else
      \global\advance\@nameuse{c@\@captype}\m@ne
    \fi
  \egroup}
\newcommand*{\@subfigcaptionlist}{}
\newcommand{\@subcaption}[3]{%
  \ifx \relax#2\relax \else
    \bgroup
      \let\label=\@gobble
      \let\protect=\string
      \def\@subcaplabel{\@nameuse{@@the#1}}%
      \xdef\@subfigcaptionlist{%
        \@subfigcaptionlist,%
        {\protect\numberline{\@subcaplabel}\noexpand{\ignorespaces #2}}}%
    \egroup
  \fi
  \@nameuse{@make#1caption}{\@nameuse{@the#1}}{#3}}
\newcommand*{\listsubcaptions}{%
  \@ifstar
    {\gdef\@subfigcaptionlist{}}%
    {\@listsubcaptions{\@captype}}}
\newcommand*{\@listsubcaptions}[1]{%
  \@ifundefined{@captype}{}{%
    \@ifundefined{ext@sub#1}{}{%
      \@for \sf@temp:=\@subfigcaptionlist \do {%
        \ifx \@empty\sf@temp\relax \else
          \addcontentsline
            {\@nameuse{ext@sub#1}}%
            {sub#1}%
            {\sf@temp}%
        \fi}}}%
  \gdef\@subfigcaptionlist{}}
\newcommand{\@makesubfigurecaption}[2]{%
  \setbox\@tempboxa\hbox{%
    \subcapsize
    {\subcaplabelfont #1}%
    {\subcapfont\ignorespaces #2}}%
  \@tempdimb=-\subfigcapmargin
  \multiply\@tempdimb\tw@
  \advance\@tempdimb\@tempdima
  \hbox to\@tempdima{%
    \hss
    \ifdim \wd\@tempboxa >\@tempdimb
      \subfig@caption{#1}{#2}%
    \else\ifsubcapnooneline
      \subfig@caption{#1}{#2}%
    \else
      \box\@tempboxa
    \fi\fi
    \hss}}
\let\@makesubtablecaption=\@makesubfigurecaption
\newcommand{\subfig@caption}[2]{%
  \ifsubcaphang
    \sbox{\@tempboxa}{\subcapsize\subcaplabelfont #1}%
    \addtolength{\@tempdimb}{-\wd\@tempboxa}%
    \usebox{\@tempboxa}%
    \subfig@captionpar{\@tempdimb}{%
      {\subcapfont\ignorespaces #2}}%
  \else
    \subfig@captionpar{\@tempdimb}{%
      {\subcaplabelfont #1}%
      {\subcapfont\ignorespaces #2}}%
  \fi}
\newcommand{\subfig@captionpar}[2]{%
  \parbox[t]{#1}{%
    \subcapsize
    \ifsubcapraggedright
      \setlength{\leftskip}{\z@}%
      \setlength{\@rightskip}{\@flushglue}%
      \setlength{\rightskip}{\@rightskip}%
      \setlength{\parindent}{\z@}%
    \else\ifsubcapcenter
      \setlength{\leftskip}{\@flushglue}%
      \setlength{\rightskip}{\@flushglue}%
      \setlength{\parfillskip}{\z@skip}%
    \else\ifsubcapcenterlast
      \addtolength{\leftskip}{\z@ plus 1fil}%
      \addtolength{\rightskip}{\z@ plus -1fil}%
      \setlength{\parfillskip}{\z@ plus 2fil}%
    \fi\fi\fi
    #2}}
\newcommand*{\@dottedxxxline}[6]{%
  \ifnum #2>\@nameuse{c@#1depth}\else
    \@dottedtocline{0}{#3}{#4}{#5}{#6}
  \fi}
\let\subfig@end@float=\end@float
\renewcommand*{\end@float}{%
  \@listsubcaptions{\@captype}%
  \subfig@end@float}
\let\subfig@end@dblfloat=\end@dblfloat
\renewcommand*{\end@dblfloat}{%
  \@listsubcaptions{\@captype}%
  \subfig@end@dblfloat}
\let\subfig@oldcaption=\@caption
\long\def\@caption#1[#2]#3{%
  \@ifundefined{if#1topcap}%
    {\subfig@oldcaption{#1}[{#2}]{#3}}%
    {\@nameuse{if#1topcap}%
       \@listsubcaptions{#1}%
       \subfig@oldcaption{#1}[{#2}]{#3}%
     \else
       \subfig@oldcaption{#1}[{#2}]{#3}%
       \@listsubcaptions{#1}%
     \fi}}
\let\subfig@oldlabel=\relax
\newcommand*{\subfloat@label}{%
  \@ifnextchar(
    {\sf@sub@label}
    {\sf@sub@label(Sub\@captype\space
                   \@ifundefined{thechapter}{}{%
                     \@nameuse{thechapter}\space}%
                   \@nameuse{p@sub\@captype}%
                   \@nameuse{thesub\@captype}.)}}
\let\sub@label\subfloat@label
\def\sf@sub@label(#1)#2{%
  \ifhyperrefloaded
    \protected@edef\@currentlabelname{%
      \expandafter\strip@period #1\relax.\relax\@@@}%
  \fi
  \sf@@sub@label{#2}}
\newcommand*{\sf@@sub@label}[1]{%
  \@bsphack
  \subfig@oldlabel{#1}%
  \ifhyperrefloaded
    \protected@write\@auxout{}{%
        \string\newlabel{sub@#1}%
            {{\@nameuse{@@thesub\@captype}}%
            {\thepage}%
            {\expandafter\strip@period\@currentlabelname\relax.\relax\@@@}%
            {\@currentHref}%
            {}}}%
  \else
    \protected@write\@auxout{}{%
        \string\newlabel{sub@#1}%
            {{\@nameuse{@@thesub\@captype}}%
            {\thepage}}}%
  \fi
  \@esphack}
\newcommand\subref[1]{%
  \ref{sub@#1}}
\newcommand\Subref[1]{%
  {\subcaplabelfont
   \ref{sub@#1}}}
\endinput
%%
%% End of file `subfigure.sty'.

